Visualizing How Embeddings Generalize

Deep metric learning is often used to learn an embedding function that captures the semantic differences within a dataset. A key factor in many problem domains is how this embedding generalizes to new classes of data. In observing many triplet selection strategies for Metric Learning, we find that the best performance consistently arises from approaches that focus on a few, well selected triplets.We introduce visualization tools to illustrate how an embedding generalizes beyond measuring accuracy on validation data, and we illustrate the behavior of a range of triplet selection strategies.

==> figs/cub_tsne.tex <==
\begin{figure}[ht]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
	 \begin{subfigure}[]{\columnwidth}
	    \begin{subfigure}[]{.3\columnwidth}
	        \caption{Train}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/BatchAll/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \caption{Test}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/BatchAll/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \caption{Train+Test}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/BatchAll/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_ba}\textit{Batch All}}
	 \end{subfigure}
	 \\
	 \begin{subfigure}[]{\columnwidth}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/Npair/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/Npair/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/Npair/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_npair}\textit{Npair}}
	 \end{subfigure}
	 \\
	 \begin{subfigure}[]{\columnwidth}
	    
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/SHN/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/SHN/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/SHN/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_shn}\textit{Random Positive Semi-Hard Negative}}
	 \end{subfigure}
	 \\
	 \begin{subfigure}[]{\columnwidth}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/EPSHN/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/EPSHN/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/cub/fc/EPSHN/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_epshn}\textit{Easy Positive Semi-Hard Negative}}
	 \end{subfigure}
	 \caption{t-SNE visualizations of different embedding approaches on the CUB dataset, showing the embedding of the training (left) and testing (center) categories to highlight their structure, and a joint embedding of the training and the testing classes (right) to highlight where test data (blue) embeds relative to training data (red).}
	 \label{fig:cub_tsne}
\end{figure}

==> figs/front_page.tex <==
\begin{figure}[t]
    \centering
    \captionsetup[subfigure]{labelformat=empty}
	 \begin{subfigure}[]{\columnwidth}
	    \begin{subfigure}[]{.3\columnwidth}
	        \caption{Train}
	        \vspace{-0.05in}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/BatchAll/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \caption{Test}
	        \vspace{-0.05in}	        \includegraphics[width=\columnwidth]{figs/tsne/fc/BatchAll/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \caption{Train+Test}
	        \vspace{-0.05in}	        \includegraphics[width=\columnwidth]{figs/tsne/fc/BatchAll/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_ba}\textit{Batch All}}
	 \end{subfigure}
     \\
	 \begin{subfigure}[]{\columnwidth}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/Npair/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/Npair/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/Npair/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_npair}\textit{Npair}}
	 \end{subfigure}
	 \\
	 \begin{subfigure}[]{\columnwidth}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/SHN/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/SHN/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/SHN/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_shn}\textit{Random Positive Semi-Hard Negative}}
	 \end{subfigure}
	 \\
	 \begin{subfigure}[]{\columnwidth}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/EPSHN/train.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/EPSHN/test.jpg}
	    \end{subfigure}
	    \begin{subfigure}[]{.3\columnwidth}
	        \includegraphics[width=\columnwidth]{figs/tsne/fc/EPSHN/combined.jpg}
	    \end{subfigure}
	    \caption{\label{fig:tsne_fc_epshn}\textit{Easy Positive Semi-Hard Negative}}
	 \end{subfigure}
    \caption{We introduce several visualizations to characterize how embeddings generalize to new data.  For the CAR dataset embedding with NPairs (a,b,c) are a jointly-embedding t-SNE showing (a) training data, (b) test data, and (c) both together, collectively, these show where how the test data is embedded relative to the training data.  At a finer scale, scatter plots showing the distance to the most similar example from the same and different classes in (d) training and (e) testing data, highlight that nPairs may fail to generalize to new classes because new class images may not be embedded to similar locations.  (f) shows histograms of distance to all same and different class pairs in the training and test sets.}
}
\label{fig:front_page}
\end{figure}

==> figs/fullpagecuborig.tex <==
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{.5}
\begin{figure*}[h]
    \centering
    \begin{tabular}{ccccccc}
        \centering
        & \parbox{1.5cm}{\raggedright \centering t-SNE\\ (train)}
        & \parbox{1.5cm}{\raggedright \centering t-SNE\\ (test)} 
        & \parbox{1.5cm}{\raggedright \centering t-SNE\\ (combined)} 
        & \parbox{1.5cm}{\raggedright \centering scatter\\ (train)} 
        & \parbox{1.5cm}{\raggedright \centering scatter\\ (test)}\\
        
        \raisebox{.7cm}{\rotatebox{90}{Batch-All}} & 
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/BatchAll/train.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/BatchAll/test.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/BatchAll/combined.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/train/ba.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/test/ba.jpg}
        
        \\
        
        \raisebox{1cm}{\rotatebox{90}{N-pair}} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/Npair/train.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/Npair/test.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/Npair/combined.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/train/npair.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/test/npair.jpg}

        \\
        
        \raisebox{1.1cm}{\rotatebox{90}{SHN}} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/SHN/train.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/SHN/test.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/SHN/combined.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/train/shn.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/test/shn.jpg}
        
        \\
        
        \raisebox{.8cm}{\rotatebox{90}{EPSHN}} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/EPSHN/train.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/EPSHN/test.jpg} &
        \includegraphics[natwidth=5960,natheight=6600]{figs/tsne/cub/fc/EPSHN/combined.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/train/epshn.jpg} &
        \includegraphics[natwidth=460,natheight=460]{figs/scatter_CUB_WT/fc/test/epshn.jpg}
    \end{tabular}
    \caption{For each embedding approach, we show the joint t-SNE embedding of training and test data from the CUB dataset~\cite{CUB200}, and both together (training data in red, testing data in blue); collectively, these show how the test data is embedded relative to the training data. The scatter plots showing the distance to the most similar example from the same and different classes in training and testing data. Examples that are closer to a same class result are colored in cyan, while examples that are closer to a different class result are color in orange.}
\label{fig:full_page}
\end{figure*}

==> figs/scatter.tex <==
\newcommand{\rulesep}{\unskip\ \vrule\ }
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\columnwidth}
    \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/train/ba.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/test/ba.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/train/ba.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/test/ba.jpg}
	    \caption{Batch All}
	\end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/train/npair.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/test/npair.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/train/npair.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/test/npair.jpg}
	    \caption{Npair}
	\end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/train/epshn.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/test/epshn.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/train/epshn.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/test/epshn.jpg}
	    \caption{Easy Positive Semi-Hard Negative}
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
        \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/train/shn.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/test/shn.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/train/shn.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/test/shn.jpg}
	    \caption{Random Positive Semi-Hard Negative (fc)}
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
        \centering
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/train/shn.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter/fc/test/shn.jpg}
	   % \\
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/train/shn.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter/pooling/test/shn.jpg}
	    \caption{Random Positive Semi-Hard Negative (pooling)}
	\end{subfigure}
	\caption{Scatter plot of different embedding approaches, showing similarity (dot product) of each instance with its easiest positive (blue) and its hardest negative (red)}
\end{figure}

==> figs/scatter_CUB.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\columnwidth}
    \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/train/ba.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/test/ba.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/train/ba.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/test/ba.jpg}
	    \caption{Batch All}
	\end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/train/npair.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/test/npair.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/train/npair.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/test/npair.jpg}
	    \caption{Npair}
	\end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
        \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/train/epshn.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/test/epshn.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/train/epshn.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/test/epshn.jpg}
	    \caption{Easy Positive Semi-Hard Negative}
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
        \centering
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/train/shn.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/test/shn.jpg}
	   % \\
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/train/shn.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/test/shn.jpg}
	    \caption{Random Positive Semi-Hard Negative (fc)}
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
        \centering
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/train/shn.jpg}
	   % \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/fc/test/shn.jpg}
	   % \\
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/train/shn.jpg}
	    \includegraphics[width=0.4\columnwidth]{figs/scatter_CUB/pooling/test/shn.jpg}
	    \caption{Random Positive Semi-Hard Negative (pooling)}
	\end{subfigure}
	\caption{Scatter plot of different embedding approaches in CUB dataset, showing similarity (dot product) of each instance with its easiest positive(cyan) instance and its hardest negative(orange) instance}
\end{figure}
